Model Identification Adaptive Control with $\rho$-POMDP Planning

Accurate system modeling is crucial for safe, effective control, as misidentification can lead to accumulated errors, especially under partial observability. We address this problem by formulating informative input design and model identification adaptive control (MIAC) as belief space planning problems, modeled as partially observable Markov decision processes with belief-dependent rewards ($\rho$-POMDPs). We treat system parameters as hidden state variables that must be localized while simultaneously controlling the system. We solve this problem with an adapted belief-space iterative Linear Quadratic Regulator (BiLQR). We demonstrate it on fully and partially observable tasks for cart-pole and steady aircraft flight domains. Our method outperforms baselines such as regression, filtering, and local optimal control methods, even under instantaneous disturbances to system parameters.

==> algs/kf.tex <==
\begin{algorithm}
\caption{Extended Kalman Filter Update}\label{alg:cap}
\begin{algorithmic}
\begin{align*}
T(s' \mid s, \mathbf{a}) &= \mathcal{N}(s' \mid \mathbf{f}_T(s, \mathbf{a}), \Sigma_s) \\
O(\mathbf{o} \mid s') &= \mathcal{N}(\mathbf{o} \mid \mathbf{f}_O(s'), \Sigma_o)
\end{align*}
\begin{align*}
\mu_p &\leftarrow \mathbf{f}_T(\mu_b, \mathbf{a}) \\
\mathbf{T}_s &= \text{jacobian}(s \rightarrow \mathbf{f}_T(s, \mathbf{a}), \mu_b) \\
\mathbf{O}_s &= \text{jacobian}(\mathbf{f}_O, \mu_p) \\
\Sigma_p &\leftarrow \mathbf{T}_s \Sigma_b \mathbf{T}_s^\top + \Sigma_s
\end{align*}
\begin{align*}
\mathbf{K} &\leftarrow \Sigma_p \mathbf{O}_s^\top \left( \mathbf{O}_s \Sigma_p \mathbf{O}_s^\top + \Sigma_o \right)^{-1} \\
\mu_b &\leftarrow \mu_p + \mathbf{K}(\mathbf{o} - \mathbf{O}_s \mu_p) \\
\Sigma_b &\leftarrow (\mathbf{I} - \mathbf{K} \mathbf{O}_s) \Sigma_p
\end{align*}
\end{algorithmic}
\end{algorithm}

==> algs/platt_alg.tex <==

\begin{algorithm}

\caption{Platt Algorithm}\label{alg:platt}
\textbf{Input}: initial belief state, $b$. \\
\textbf{Output}: vector of control actions, $u_{1:T}$.
   \begin{algorithmic}
\While{ $b$ not at goal} \do \\
    \State $(\bar{u}_{1:T}, \bar{b}_{1:T}) = \texttt{create\_plan}(b);$
    \For{$t \gets 1$ \textbf{to} $T - 1$} \do \\
        \State $u_t = \texttt{lqr\_control}(b_t, \bar{u}_t, \bar{b}_t);$
        \State $b_{t+1} = \texttt{EKF}(b_t, u_t, z_t);$
        \If{$\tilde{m}_{t+1} > \theta$}
            \State \textbf{break;}
        \EndIf
    \State $b = b_{t+1};$
    \EndFor 
\EndWhile

\end{algorithmic} 
\end{algorithm}

==> sections/06-acknowledgements.tex <==
% \section*{Acknowledgments}

% This material is based upon work supported by the National Science Foundation Graduate Research Fellowship Program under Grant No. DGE-1656518. 
% %Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation. 
% % This work is also supported by the COMET K2---Competence Centers for Excellent Technologies Programme of the Federal Ministry for Transport, Innovation and Technology (bmvit), the Federal Ministry for Digital, Business and Enterprise (bmdw), the Austrian Research Promotion Agency (FFG), the Province of Styria, and the Styrian Business Promotion Agency (SFG). The authors would also like to acknowledge the funding support from OMV.

==> sections/99_01_proofs.tex <==
\subsection{Proofs from THE KYLE}

When options are feasible when executed under a budget for their decision epoch, \algname\ can maintain feasibility.
To show this, we first define the concept of a locally feasible option in~\cref{def_appendix:locally-feasible-option} below.
Informally, such an option ensures it does not go over a budget set while it is in control.

\begin{definition}
    \label{def_appendix:locally-feasible-option}
    For an option $\hat{a}_\ep$ chosen at decision epoch $e$ in $b_\ep$, given budget $\hat{\mathbf{c}}_\ep$, is \emph{locally feasible} if $\mathbf{Q}_\mathbf{C}^\pi(b_\ep, \hat{a}_\ep) \leq \hat{\mathbf{c}}_e$.
\end{definition}

Two additional types of feasibility, one-step global and global, are stated in Definitions~\ref{def_appendix:one-step-global-feasibility} and~\ref{def_appendix:global-feasibility}, respectively.
Informally, the first describes an option that can be applied once and guarantee it does not go over the allotted budget.

\begin{definition}
    \label{def_appendix:one-step-global-feasibility}
    An option $\hat{a}_\ep$ chosen at decision epoch $\ep$ in $b_\ep$ is \emph{one-step globally feasible} if $\tilde{\mathbf{c}}_{\ep-1} + \mathbf{Q}_{\mathbf{C},\ep}^\pi(b_\ep, \hat{a}_\ep) \leq \hat{\mathbf{c}}$.
\end{definition}

This second definition states that an agent is globally feasible if the original constraints from~\cref{eq:cpomdp-objective-constraints} are satisfied.

\begin{definition}
    \label{def_appendix:global-feasibility}
    An algorithm or policy $\pi$ is said to be \emph{globally feasible} if $\mathbf{V}_{\mathbf{C}}^\pi(b_0) \leq \hat{\mathbf{c}}$.
\end{definition}

With these definitions,~\cref{prop_appen:local-feasible-option-with-hatct-one-step-globally-feasible} below shows that for a CPOSMDP, if a locally feasible option is chosen with a particular assignment of $\hat{\mathbf{c}}_\ep$, then it ensures that one-step is globally feasible.

\begin{proposition}
    \label{prop_appen:local-feasible-option-with-hatct-one-step-globally-feasible}
    For policy $\pi$ and locally feasible option $\hat{a}_\ep$, if $\hat{\mathbf{c}}_\ep$ = $\frac{\hat{\mathbf{c}} - \tilde{\mathbf{c}}_{\ep-1}}{\gamma^{t_{\ep-1}}} \geq 0$ with $\tilde{\mathbf{c}}_0 = \mathbf{0}$ at decision epoch $\ep$, which is at time $t_{\ep-1}$ and accumulated costs $\tilde{c}_{\ep-1}$, then $\hat{a}_\ep$ is one-step globally feasible.
\end{proposition}

\begin{proof}
By definition of a locally feasible option and the choice of $\hat{\mathbf{c}}_e$:
\begin{align*}
    &\mathbf{Q}_{\mathbf{C}}(b_\ep, \hat{a}_\ep) \leq \hat{\mathbf{c}}_\ep \\
    &\mathbb{E}\Big[\sum_{i=0}^\infty \gamma^i \mathbf{C}(b_i', a_i') | b_0' {=} b_\ep, a_0' {=} \hat{a}_\ep, \pi \Big] \leq \hat{\mathbf{c}}_\ep \\
    &\mathbb{E}\Big[\sum_{j=t_{\ep-1}}^\infty \gamma^{i-t_{\ep-1}} \mathbf{C}(b_j, a_j) | b_{t_{\ep-1}} {=} b_\ep, a_{t_{\ep-1}} {=} \hat{a}_\ep, \pi \Big] \leq \hat{\mathbf{c}}_\ep \\
    %&\mathbb{E}\Big[\sum_{j=t_{\ep-1}}^\infty \gamma^{i-t_{\ep-1}} \mathbf{C}(b_j, a_j) | b_{t_{\ep-1}} = b_\ep, a_{t_{\ep-1}} = \hat{a}_\ep, \pi \Big] \leq \frac{\hat{\mathbf{c}} - \tilde{\mathbf{c}}_{\ep-1}}{\gamma^{t_{\ep-1}}} \\
    &\mathbb{E}\Big[\sum_{j=t_{\ep-1}}^\infty \gamma^{i-t_{\ep-1}} \mathbf{C}(b_j, a_j) | \text{---} \Big] \leq \frac{\hat{\mathbf{c}} - \tilde{\mathbf{c}}_{\ep-1}}{\gamma^{t_{\ep-1}}} \\
    %&\tilde{\mathbf{c}}_{\ep-1} + \gamma^{t_{\ep-1}} \mathbb{E}\Big[\sum_{j=t_{\ep-1}}^\infty \gamma^{i-t_{\ep-1}} \mathbf{C}(b_j, a_j) | b_{t_{\ep-1}} = b_\ep, a_{t_{\ep-1}} = \hat{a}_\ep, \pi \Big] \leq \hat{\mathbf{c}} \\
    &\tilde{\mathbf{c}}_{\ep-1} + \gamma^{t_{\ep-1}} \mathbb{E}\Big[\sum_{j=t_{\ep-1}}^\infty \gamma^{i-t_{\ep-1}} \mathbf{C}(b_j, a_j) | \text{---} \Big] \leq \hat{\mathbf{c}} \\
    %&\tilde{\mathbf{c}}_{\ep-1} + \mathbb{E}\Big[\sum_{j=t_{\ep-1}}^\infty \gamma^{i} \mathbf{C}(b_j, a_j) | b_{t_{\ep-1}} = b_\ep, a_{t_{\ep-1}} = \hat{a}_\ep, \pi \Big] \leq \hat{\mathbf{c}} \\
    &\tilde{\mathbf{c}}_{\ep-1} + \mathbb{E}\Big[\sum_{j=t_{\ep-1}}^\infty \gamma^{i} \mathbf{C}(b_j, a_j) | \text{---} \Big] \leq \hat{\mathbf{c}} \\
    &\tilde{\mathbf{c}}_{\ep-1} + \mathbf{Q}_{\mathbf{C},t}^\pi(b_\ep, \hat{a}_\ep) \leq \hat{\mathbf{c}} \text{.}
\end{align*}
Thus, by~\cref{def_appendix:one-step-global-feasibility}, $\hat{a}_e$ is one-step globally feasible.
\end{proof}

Combining these results yields that \algname\ is globally feasible when its options are one-step globally feasible.

\begin{proposition}
    \label{prop_appen:cobets-globally-feasible}
    \algname\ is globally feasible if all its options $\hat{a}_e$ are locally feasible given \algname\ dynamic assignments of $\hat{\mathbf{c}}_\ep \geq 0$ for all $\ep$.
\end{proposition}

\begin{proof}
By construction.
Consider any decision epoch $\ep$.
As given, consider any \algname\ option $\hat{a}_\ep$.
By definition of \algname, it assigns $\hat{\mathbf{c}}_\ep = \frac{\hat{\mathbf{c}} - \tilde{\mathbf{c}}_{\ep-1}}{\gamma^{t_{\ep-1}}} \geq 0$.
By~\cref{prop_appen:local-feasible-option-with-hatct-one-step-globally-feasible}, it is one-step globally feasible.
Since this is true for $\ep$, \algname\ is globally feasible.
\end{proof}

==> sections/99_02_domains.tex <==
\subsection{Domains}

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figs/roomba.png}
\caption{In the Roomba CPOMDP environments, the robot must localize its belief (blue) before navigating to the goal region (green) while avoiding the penalty region (red line) and constrained regions (red box).}
\label{fig:roomba}
\end{figure}

==> tables/miac_results_4.tex <==



\begin{tabular}{@{}r ccc ccc ccc ccc @{}} 
\toprule
& \multicolumn{3}{c}{\textbf{Cart-Pole Full Obs}} 
& \multicolumn{3}{c}{\textbf{Cart-Pole Partial Obs}} 
& \multicolumn{3}{c}{\textbf{Aircraft Full Obs}} 
& \multicolumn{3}{c}{\textbf{Aircraft Partial Obs}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
\textbf{Solver} &
{$\mathrm{tr}(\Sigma_{\param\param,\hor})$} & {$\log{p_{\param,\hor}}$} & $ R(b,a)$ & 
{$\mathrm{tr}(\Sigma_{\param\param,\hor})$} & {$\log{p_{\param,\hor}}$} & $ R(b,a)$ & 
{$\mathrm{tr}(\Sigma_{\param\param,\hor})$} & {$\log{p_{\param,\hor}}$} & $ R(b,a)$ & 
{$\mathrm{tr}(\Sigma_{\param\param,\hor})$} & {$\log{p_{\param,\hor}}$} & $ R(b,a)$ \\
\midrule 

\texttt{BiLQR} &
$0.0104 \scriptstyle\pm 0.0008$ &
$0.0224 \scriptstyle\pm 0.3275$ & 
$4.2508 \scriptstyle\pm 2.0501$ &
$0.1403 \scriptstyle\pm 0.0100$ &
$-0.6988 \scriptstyle\pm 0.1693$ & 
$4.0348 \scriptstyle\pm 2.0459$ &
$2.0574 \scriptstyle\pm 0.1196 $ & 
$-3.3769 \scriptstyle\pm 3.3533 $ & 
$ 77.9533 \scriptstyle \pm 12.9046$ &
$22.6091 \scriptstyle\pm 0.3343 $ &
$-7.9188 \scriptstyle\pm 0.8997$ & 
$78.4286 \scriptstyle \pm 12.4708 $ \\

\texttt{MPC + Regression} &
$0.0963 \scriptstyle\pm 0.0109 $ & 
$-46.6712 \scriptstyle\pm 6.2698$ & 
$3.6867 \scriptstyle\pm 1.6350 $ &
- & - & - &

$44.9742 \scriptstyle\pm 0.2892$ & 
$-180.0136 \scriptstyle \pm 10.1276$ &
$3.7067 \scriptstyle \pm 0.9015 $ &
$ - $ & $ - $ & $-$ \\

\texttt{MPC + EKF} &
$0.0108 \scriptstyle\pm 0.0012 $ & 
$-6.4969 \scriptstyle\pm 5.1016 $ & 
$3.7477 \scriptstyle\pm 2.1849 $ &
$0.1449 \scriptstyle\pm 0.0102$ & 
$-13.1135 \scriptstyle\pm 9.7824$ & 
$3.8632 \scriptstyle\pm 2.0523$ &
$9.440 \scriptstyle\pm 0.2123 $ & 
$-7.5777 \scriptstyle\pm 3.0101$ & 
$56.0400 \scriptstyle \pm 18.2392$ &
$20.7412 \scriptstyle\pm 0.1458$ & 
$-8.0349 \scriptstyle\pm 6.2883$ & 
$58.0333 \scriptstyle \pm 19.2418$ \\

\texttt{EKF} &
$0.0215 \scriptstyle\pm 0.0022$ & 
$-39.9446 \scriptstyle\pm 29.8609$ &  
$3.5836 \scriptstyle\pm 1.8039$ &
$0.1320 \scriptstyle\pm 0.0109 $ & 
$-4.4754 \scriptstyle\pm 2.9213$ & 
$3.6060 \scriptstyle\pm 2.1406$ &
$32.3293 \scriptstyle\pm 0.14789$ & 
$-31.2193 \scriptstyle\pm 2.6128$ & 
$51.7067 \scriptstyle \pm 17.3052$ &
$45.9700 \scriptstyle\pm 0.0786$ & 
$-17.8365 \scriptstyle\pm 1.9365$ & 
$51.9667 \scriptstyle \pm 16.6783$ \\

\bottomrule
\end{tabular}




==> tables/old.tex <==
\scalebox{0.85}{ % Adjust the scale factor as needed
\begin{tabular}{@{}r RRRRRRRR @{}}
\toprule
&\multicolumn{2}{c}{\underline{\quad\quad\textbf{Cart-Pole Full Obs}\quad\quad}}
&\multicolumn{2}{c}{\underline{\quad\quad\textbf{Cart-Pole Partial Obs}\quad\quad}}
&\multicolumn{2}{c}{\underline{\quad\quad\quad\textbf{Aircraft Full Obs}\quad\quad\quad}}
&\multicolumn{2}{c}{\underline{\quad\quad\quad\textbf{Aircraft Partial Obs}\quad\quad\quad}}\\
\textbf{Solver} &  
{tr(\Sigma_{\param \param,T})} & {\log{p_{\param,T}}} & 
{tr(\Sigma_{\param \param,T})} & {\log{p_{\param,T}}} & 
{tr(\Sigma_{\param \param,T})} & {\log{p_{\param,T}}} & 
{tr(\Sigma_{\param \param,T})} & {\log{p_{\param,T}}} \\
\midrule
\texttt{BiLQR}           &  
(5.9920 \scriptstyle\pm 0.3421)\times \num{e-5} & 3.4335 \scriptstyle\pm 0.7979 &  
(0.0115 \scriptstyle\pm 0.0015 )\times \num{e-5} & -12.4437 \scriptstyle\pm  59.3036 &  
0.0178 \scriptstyle\pm 0.0089 & 23.4029 \scriptstyle\pm 6.5601 &  
4.1756 \scriptstyle\pm 0.0737 & 0.8612 \scriptstyle\pm 0.8356 \\
\texttt{EKF}           &  
(23.0850 \scriptstyle\pm 3.8901) \times \num{e-5} & 2.9285 \scriptstyle\pm 1.0059 &  
(0.0131\scriptstyle\pm0.0019) \times \num{e-5} & -65.3207 \scriptstyle\pm 258.2325 &  
0.2282 \scriptstyle\pm 0.0128 & 23.6622 \scriptstyle\pm 17.6774 &  
4.2100 \scriptstyle\pm 0.0141 & 0.5628 \scriptstyle\pm 1.2501 \\
\texttt{Regression}            &  
(473.6769\scriptstyle\pm11.5723)\num{e-5} & -290.2938 \scriptstyle\pm 280.7291 &  
- & - &  
(3.2198 \scriptstyle\pm 3.8901) \times \num{e35} & (3.2198 \scriptstyle\pm 3.8901) \times \num{e35} &  
- & - \\
\bottomrule
\end{tabular}
}


\scalebox{0.85}{ 


\begin{tabular}{@{}r ccc ccc ccc ccc @{}} 
\toprule
& \multicolumn{3}{c}{\textbf{Cart-Pole Full Obs}} 
& \multicolumn{3}{c}{\textbf{Cart-Pole Partial Obs}} 
& \multicolumn{3}{c}{\textbf{Aircraft Full Obs}} 
& \multicolumn{3}{c}{\textbf{Aircraft Partial Obs}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
\textbf{Solver} &
{$\mathrm{tr}(\Sigma_{\param\param, T})$} & {$\log{p_{\param, T}}$} & {$\mathbb{E}[R(b,a)]$} & 
{$\mathrm{tr}(\Sigma_{\param\param, T})$} & {$\log{p_{\param, T}}$} & {$\mathbb{E}[R(b,a)]$} & 
{$\mathrm{tr}(\Sigma_{\param\param, T})$} & {$\log{p_{\param, T}}$} & {$\mathbb{E}[R(b,a)]$} & 
{$\mathrm{tr}(\Sigma_{\param\param, T})$} & {$\log{p_{\param, T}}$} & {$\mathbb{E}[R(b,a)]$} \\
\midrule 
\texttt{BiLQR} &
$(53.25 \pm 9.66) \times 10^{-5}$ & $3.0720 \pm 1.0550$ & $8.9667 \pm 0.2582$ &
$0.0142 \pm 0.0016$ & $-0.30 \pm 2.29$ & $5.2143 \pm 0.6242$ &
$0 \pm 0$ & $0 \pm 0$ & - &
$0 \pm 0$ & $0 \pm 0$ & - \\
\texttt{MPC + Regression} &
$(510.80 \pm 14.47) \times 10^{-5}$ & $-269.24 \pm 255.03$ & $4.9333 \pm 0.6856$ &
- & - & - &
$0 \pm 0$ & $0 \pm 0$ & - &
$0 \pm 0$ & $0 \pm 0$ & - \\
\texttt{MPC + EKF} &
$(162.23 \pm 13.91) \times 10^{-5}$ & $1.8828 \pm 0.7243$ & $8.1034 \pm 3.805$ &
$0.1389 \pm 0.0123$ & $-2.03 \pm 6.79$ & $2.500 \pm 2.1992$ &
$0 \pm 0$ & $0 \pm 0$ & - &
$0 \pm 0$ & $0 \pm 0$ & - \\
\texttt{Random + EKF} &
$(173.22 \pm 21.89) \times 10^{-5}$ & $2.0038 \pm 0.8390$ & $8.3000 \pm 3.5477$ &
$0.0117 \pm 0.0021$ & $-419.49 \pm 3096.51$ & $5.1379 \pm 0.6338$ &
$0 \pm 0$ & $0 \pm 0$ & - &
$0 \pm 0$ & $0 \pm 0$ & - \\
\bottomrule
\end{tabular}


} 

==> tables/sysid_results_4.tex <==
\scalebox{0.9}{ % Adjust the scale factor as needed
\begin{tabular}{@{}r RRRRRRRR @{}}
\toprule
&\multicolumn{2}{c}{\underline{\quad\quad\textbf{Cart-Pole Full Obs}\quad\quad}}
&\multicolumn{2}{c}{\underline{\quad\quad\textbf{Cart-Pole Partial Obs}\quad\quad}}
&\multicolumn{2}{c}{\underline{\quad\quad\quad\textbf{Aircraft Full Obs}\quad\quad\quad}}
&\multicolumn{2}{c}{\underline{\quad\quad\quad\textbf{Aircraft Partial Obs}\quad\quad\quad}}\\
\textbf{Solver} &  
{\text{tr}(\Sigma_{\param \param,\hor})} & {\log{p_{\param,\hor}}} & 
{\text{tr}} & {\log{p_{\param,\hor}}} & 
{\text{tr}(\Sigma_{\param \param,\hor})} & {\log{p_{\param,\hor}}} & 
{\text{tr}(\Sigma_{\param \param,\hor})} & {\log{p_{\param,\hor}}} \\
\midrule
\texttt{BiLQR}           &  
0.0120 \scriptstyle \pm 0.0012 & 
0.5135 \scriptstyle\pm 0.1474 &
0.1083 \scriptstyle\pm 0.0074 & 
-2.3955 \scriptstyle\pm  1.8239 &  
7.9941 \scriptstyle\pm 0.4699 & 
-4.9763 \scriptstyle\pm 0.4246 &
22.6044 \scriptstyle\pm 0.8157 & 
-7.7919 \scriptstyle\pm 1.2021\\

\texttt{EKF}           &  
0.0215 \scriptstyle\pm 0.0022 & 
-39.9446 \scriptstyle\pm 29.8609 &  
0.1320 \scriptstyle\pm 0.0109 & 
-4.5073 \scriptstyle\pm 2.9317 &  
32.3293 \scriptstyle\pm 0.14789 & 
-31.2193 \scriptstyle\pm 2.6128 & 
45.9700 \scriptstyle\pm 0.0786 & 
-17.8365 \scriptstyle\pm 1.9365 \\

\texttt{Regression}            &  
0.1721 \scriptstyle \pm 0.0812 & 
-35.2348 \scriptstyle\pm 3.9663  &  
- & - &  
49.4794 \scriptstyle \pm 0.2337 & 
-28.8654 \scriptstyle \pm 1.3617 &  
- & - \\
\bottomrule
\end{tabular}
}

